Constructing Holistic Spatio-Temporal Scene Graph for Video Semantic Role Labeling

Video Semantic Role Labeling (VidSRL) aims to detect the salient events from given videos, by recognizing the predict-argument event structures and the interrelationships between events. While recent endeavors have put forth methods for VidSRL, they can be mostly subject to two key drawbacks, including the lack of fine-grained spatial scene perception and the insufficiently modeling of video temporality. Towards this end, this work explores a novel holistic spatio-temporal scene graph (namely HostSG) representation based on the existing dynamic scene graph structures, which well model both the fine-grained spatial semantics and temporal dynamics of videos for VidSRL. Built upon the HostSG, we present a nichetargeting VidSRL framework. A scene-event mapping mechanism is first designed to bridge the gap between the underlying scene structure and the high-level event semantic structure, resulting in an overall hierarchical scene-event (termed ICE) graph structure. We further perform iterative structure refinement to optimize the ICE graph, such that the overall structure representation can best coincide with end task demand. Finally, three subtask predictions of VidSRL are jointly decoded, where the end-to-end paradigm effectively avoids error propagation. On the benchmark dataset, our framework boosts significantly over the current best-performing model. Further analyses are shown for a better understanding of the advances of our methods.

==> figures/app_obj_dist.tex <==
% \pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.7)}}}
\pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.45)}, font=\fontsize{14}{1}\selectfont},every axis/.append style={xtick pos=left,ytick pos=left,tickwidth=1.5pt}}
\usetikzlibrary{matrix}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns,backgrounds}

\definecolor{c1}{RGB}{252,232,212}
\definecolor{c2}{RGB}{184,183,163}
\definecolor{c3}{RGB}{107,112,092}
\definecolor{c4}{RGB}{203,153,126}
\definecolor{c5}{RGB}{107,112,092}

\begin{figure*}[t]
\centering
\begin{tikzpicture}
%\begin{groupplot}[group style={group name=myplot,group size=2 by 1,horizontal sep=30pt,xlabels at=edge bottom, ylabels at=edge left},height=4cm,width=4cm]
\begin{axis}[
	ybar,
	ytick = {60000, 111000, 162000, 213000},
	yticklabels={60000, 111000, 162000, 213000},
	ymax=213000,ymin=60000,
	% ylabel = BLEU-4,
	y tick label style = {yshift=-0.5em, text height=0ex,font=\scriptsize},
	%    ytick style = {yshift=-0.0em, font=\scriptsize},
    x label style = {font=\scriptsize},
    y label style = {yshift=-0.5em,font=\scriptsize},
	axis line style={-},
    axis x line*=bottom,
    axis y line*=left,
	enlargelimits=0.05,
	legend style={at={(0.02,0.99)},anchor=north west, draw=none, legend columns=-1, font=\scriptsize},
	xticklabels={shirt, hair, man, window, door, head, arm, hand, face, logo, letter, person, tree, ear, woman, jacket, light, eye, leg, nose},
	xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
	xmax=20, xmin=1,
	x tick label style = {yshift=0.05em,rotate=90, align=center,font=\small},
%	title=(a) BLEU-4,
	title style={yshift=-0.9em,font=\small},
    ymajorgrids,
	width = \textwidth,
	height = 5cm,
	]
	\addplot[c4, pattern= north east lines, thick, pattern color=c4, bar shift=0pt, bar width = 1em] coordinates
	{
	(1,212865)
        (2,200591)
        (3,175160)
        (4,167122)
        (5,164838)
        (6,161899)
        (7,134113)
        (8,133082)
        (9,113024)
        (10,112805)
        (11,112567)
        (12,106547)
        (13,96023)
        (14,84997)
        (15,84090)
        (16,76697)
        (17,72665)
        (18,70937)
        (19,68409)
        (20,61427)
	};

    % \addplot[c2, pattern= north east lines, thick, pattern color=c2, bar shift=0pt, bar width = 1em] coordinates
	% {
	% 	(2,  26.23)
	% };
	
	% \addplot[c3, pattern=crosshatch, pattern color=c3, thick, bar shift=0pt, bar width = 1em] coordinates
	% {
	% 	(2.7,  26.40)
	% };
\end{axis}

\end{tikzpicture}
\caption{Top 20 objects distribution in VidSRL dataset.}
\label{fig:tag_dist}
\end{figure*}


==> tables/arguments.tex <==
\begin{table}[t]
\fontsize{8}{10}\selectfont
\setlength{\tabcolsep}{1.mm}
\renewcommand\arraystretch{0.6}
\begin{center}
\caption{List of the pre-defined arguments.
% from 3D scene extractor.
}
\vspace{-3mm}
\begin{tabular}{ll}
\hline
\multirow{2}{*}{Arg0(Agent)} & \multirow{2}{*}{Object performing the action.}\\ \\
\multirow{2}{*}{Arg1(Patient)} & \multirow{2}{*}{Object on which action is performed}\\ \\
\multirow{2}{*}{Arg2} & \multirow{2}{*}{Instrument, Benefactive, Attribute} \\ \\
\multirow{2}{*}{Arg3(Start)} & \multirow{2}{*}{Starting Point} \\ \\
\multirow{2}{*}{Arg4(End)} & \multirow{2}{*}{Ending Point} \\ \\
\multirow{2}{*}{ArgM(Modifier)} & \multirow{2}{*}{location, manner, purpose, goal, direction} \\ \\
\hline
\end{tabular}
\label{tab:args}
\end{center}
\end{table}

==> tables/dataset.tex <==
\begin{table}[t]
\fontsize{8}{11}\selectfont
% \setlength{\tabcolsep}{1.mm}
% \renewcommand\arraystretch{0.6}
\begin{center}
\caption{Dataset statistics.
% from 3D scene extractor.
}
\vspace{-3mm}
\begin{tabular}{ccccc}
\hline
& Train & Valid & Test-Verb & Test-Reol \\
\hline
Clip & 118130 & 6630 & 6765 & 7990\\ 
Verb & 118130 & 66300 & 67650 & 79900\\ 
Role & 118130 & 19890 & 20295 & 23970\\ 

\hline
\end{tabular}
\label{tab:data}
\end{center}
\end{table}
